Shape model of the asteroid (2501) Lohja from long-term photometric observations

We present lightcurves, shapes, and a 3D convex spin-axis model for the main-belt asteroid (2501) Lohja. The models were obtained with the lightcurve inversion process using combined dense photometric data from the apparitions between years 2006 and 2017. The analysis found a sidereal period of 3.80835\,hours, and a possible ecliptic pole solution (J2000.0), the prograde sense of rotation and main ratios of the ellipsoidal model.

==> mybibliography <==
@ARTICLE{Harris1989,
   author = {{Harris}, A.~W. and {Young}, J.~W. and {Bowell}, E. and {Martin}, L.~J. and 
	{Millis}, R.~L. and {Poutanen}, M. and {Scaltriti}, F. and {Zappala}, V. and 
	{Schober}, H.~J. and {Debehogne}, H. and {Zeigler}, K.~W.},
    title = "{Photoelectric observations of asteroids 3, 24, 60, 261, and 863}",
  journal = "Icarus",
 keywords = {Asteroids, Electrophotometry, Light Curve, Astronomical Photometry, Fourier Analysis, ASTEROIDS, PHOTOELECTRIC METHODS, ASTRONOMY, ANALYSIS, LIGHTCURVES, ROTATION, PERIOD, MAGNITUDE, TECHNIQUES, AMPLITUDE, JUNO, THEMIS, ECHO, ALBEDO, SURFACE, EARTH-BASED OBSERVATIONS, PRYMNO, BENKOELA, PHASE RELATIONS},
     year = 1989,
    month = jan,
   volume = 77,
    pages = {171-186},
      doi = {10.1016/0019-1035(89)90015-8},
   adsurl = {http://adsabs.harvard.edu/abs/1989Icar...77..171H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KaasalainenTorppa2001,
   author = {{Kaasa\-lainen}, M. and {Torppa}, J.},
    title = "{Optimization Methods for Asteroid Lightcurve Inversion. I. Shape Determination}",
  journal = "Icarus",
     year = 2001,
    month = sep,
   volume = 153,
    pages = {24-36},
      doi = {10.1006/icar.2001.6673},
   adsurl = {http://adsabs.harvard.edu/abs/2001Icar..153...24K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KaasalainenTorppaMuinonen2001,
   author = {{Kaasalainen}, M. and {Torppa}, J. and {Muinonen}, K.},
    title = "{Optimization Methods for Asteroid Lightcurve Inversion. II. The Complete Inverse Problem}",
  journal = "Icarus",
     year = 2001,
    month = sep,
   volume = 153,
    pages = {37-51},
      doi = {10.1006/icar.2001.6674},
   adsurl = {http://adsabs.harvard.edu/abs/2001Icar..153...37K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009Icar..202..134W,
   author = {{Warner}, B.~D. and {Harris}, A.~W. and {Pravec}, P.},
    title = "{The asteroid lightcurve database}",
  journal = {Icarus},
     year = 2009,
    month = jul,
   volume = 202,
    pages = {134-146},
      doi = {10.1016/j.icarus.2009.02.003},
   adsurl = {http://adsabs.harvard.edu/abs/2009Icar..202..134W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Higgins2006,
   author = {{Higgins}, D. and {Pravec}, P. and {Kusnirak}, P. and {Galad}, A. and 
	{Kornos}, L. and {Pray}, D. and {Koff}, R.~A.},
    title = "{Asteriod lightcurve analysis at Hunters Hill Observatory and collaborating stations - autumn 2006}",
  journal = {Minor Planet Bulletin},
 keywords = {Minor Planets, Light Curves},
     year = 2006,
    month = dec,
   volume = 33,
    pages = {89-91},
   adsurl = {http://adsabs.harvard.edu/abs/2006MPBu...33...89H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HigginsOeyPravec2011,
   author = {{Higgins}, D. and {Oey}, J. and {Pravec}, P.},
    title = "{Period Determination of Binary Asteroid Targets Observed at Hunters Hill Observatory: May-September 2009}",
  journal = {Minor Planet Bulletin},
     year = 2011,
    month = jan,
   volume = 38,
    pages = {46-49},
   adsurl = {http://adsabs.harvard.edu/abs/2011MPBu...38...46H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Magnusson1989,
   author = {{Magnusson}, P. and {Barucci}, M.~A. and {Drummond}, J.~D. and 
	{Lumme}, K. and {Ostro}, S.~J. and {Surdej}, J. and {Taylor}, R.~C. and 
	{Zappal{\`a}}, V.},
    title = "{Determination of pole orientations and shapes of asteroids.}",
 keywords = {Minor Planets: Rotation, Minor Planets: Pole Coordinates, Minor Planets: Figures, Minor Planets: Light Curves},
booktitle = {Asteroids II},
     year = 1989,
   editor = {{Binzel}, R.~P. and {Gehrels}, T. and {Matthews}, M.~S.},
    pages = {66-97},
   adsurl = {http://adsabs.harvard.edu/abs/1989aste.conf...66M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Durechetal2010,
   author = {{Durech}, J. and {Sidorin}, V. and {Kaasalainen}, M.},
    title = "{DAMIT: a database of asteroid models}",
  journal = {Astron. Astrophys.},
 keywords = {minor planets, asteroids: general, astronomical data bases: miscellaneous},
     year = 2010,
    month = apr,
   volume = 513,
      eid = {A46},
    pages = {A46},
      doi = {10.1051/0004-6361/200912693},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...513A..46D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaskelletal2006,
   author = {{Gaskell}, R. and {Barnouin-Jha}, O. and {Scheeres}, D. and 
	{Mukai}, T. and {Hirata}, N. and {Abe}, S. and {Saito}, J. and 
	{Hashimoto}, T. and {Ishiguro}, M. and {Kubota}, T.},
    title = "{High Resolution Global Topography of Itokawa From Hayabusa Imaging and LIDAR Data}",
  journal = {AGU Spring Meeting Abstracts},
 keywords = {6055 Surfaces, 6205 Asteroids, 6297 Instruments and techniques},
     year = 2006,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2006AGUSM.P32A..01G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Milletetal2002,
   author = {{Miller}, J.~K. and {Konopliv}, A.~S. and {Antreasian}, P.~G. and 
	{Bordi}, J.~J. and {Chesley}, S. and {Helfrich}, C.~E. and {Owen}, W.~M. and 
	{Wang}, T.~C. and {Williams}, B.~G. and {Yeomans}, D.~K. and 
	{Scheeres}, D.~J.},
    title = "{Determination of Shape, Gravity, and Rotational State of Asteroid 433 Eros}",
  journal = {Icarus},
     year = 2002,
    month = jan,
   volume = 155,
    pages = {3-17},
      doi = {10.1006/icar.2001.6753},
   adsurl = {http://adsabs.harvard.edu/abs/2002Icar..155....3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MPBu...43...26W,
	author = {{Warner}, B.~D.},
	title = "{Save the Lightcurves! An Update on the ALCDEF Project}",
	journal = {Minor Planet Bulletin},
	year = 2016,
	month = jan,
	volume = 43,
	pages = {26-30},
	adsurl = {http://adsabs.harvard.edu/abs/2016MPBu...43...26W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2014acm..conf..225H,
	author = {{Hus\'{a}rik}, M.},
	title = "{Shapes and spins of asteroids Lohja, Ermolova, and Silver from the observations at the Skalnate Pleso Observatory}",
	booktitle = {Asteroids, Comets, Meteors 2014},
	year = 2014,
	editor = {{Muinonen}, K. and {Penttil{\"a}}, A. and {Granvik}, M. and 
	{Virkki}, A. and {Fedorets}, G. and {Wilkman}, O. and {Kohout}, T.
	},
	month = jul,
	adsurl = {http://adsabs.harvard.edu/abs/2014acm..conf..225H},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

